Can Pre-trained Language Models be Used to Resolve Textual and Semantic Merge Conflicts?

Program merging is standard practice when developers integrate their individual changes to a common code base. When the merge algorithm fails, this is called a merge conflict. The conflict either manifests in textual merge conflicts where the merge fails to produce code, or semantic merge conflicts where the merged code results in compiler or test breaks. Resolving these conflicts for large code projects is expensive because it requires developers to manually identify the sources of conflict and correct them. In this paper, we explore the feasibility of automatically repairing merge conflicts (both textual and semantic) using k-shot learning with large neural language models (LM) such as GPT-3. One of the challenges in leveraging such language models is to fit the examples and the queries within a small prompt (2048 tokens). We evaluate LMs and k-shot learning for two broad applications: (a) textual and semantic merge conflicts for a divergent fork Microsoft Edge, and (b) textual merge conflicts for a large number of JavaScript projects in GitHub. Our results are mixed: one one-hand, LMs provide the state-of-the-art (SOTA) performance on semantic merge conflict resolution for Edge compared to earlier symbolic approaches; on the other hand, LMs do not yet obviate the benefits of fine-tuning neural models (when sufficient data is available) or the design of special purpose domain-specific languages (DSL) for restricted patterns for program synthesis.

==> figs/distribution.tex <==

\begin{table}[h]
\caption{Accuracy Distribution for \app on Resolving Edge Semantic Merge Conflicts.}
\label{table:distribution}
\begin{footnotesize}
\begin{tabular}{|l|c|c|c|}
\hline
{\color[HTML]{000000} Model} & {\color[HTML]{000000} Top 1}            & {\color[HTML]{000000} Top 3}            & {\color[HTML]{000000} Top 10}                    \\ \hline
{\color[HTML]{000000} \app} & {\color[HTML]{000000} 38.8\% (147/379)} & {\color[HTML]{000000} 49.3\% (187/379)} & {\color[HTML]{000000} \textbf{64.6\% (245/379)}} \\ \hline
\end{tabular}
\end{footnotesize}
\end{table}

==> secs/experience.tex <==
\section{Experience}
\label{sec:experience}

This section aims to evaluate \app by answering the following questions: 
\begin{enumerate}
\item How effective is \app in resolving semantic merge conflicts in a divergent fork?
\item How do different choices of prompt structure, prompt content and prompt format) impact
the performance of \app?
\item How effective is \app in resolving textual merge conflicts in a divergent fork and for a large number of public JavaScript projects in GitHub.
\end{enumerate}



\subsection{Evaluate \app on semantic merge conflicts for a divergent fork}
\label{subsec:evalsemantic}

\para{Experiment Setup} 
Taking Microsoft Edge as an example, when semantic merge conflicts
We fetched all the Edge semantic merge conflicts from Aug 2020 to April 2021.
Each semantic merge conflict.

Four types of clang compiler message


% How we collect the Edge datasets? Look at the ConfigX paper to see how we collect the dataset.

% mentioning compared to the previous examples that use the human labor to classify the, we use an automatic way of handling this cases 
% Table one
% Accuracy for \app on the Edge Dataset

\para{Accuracy} The overall accuracy of \app is \accuracy, compared to the state of the art of \Astaccuracy

\input{figs/gpt3}
\input{figs/distribution}


\para {Is GPT-3 able to generate complex fix for semantic merge conflicts?} To understand how much the GPT-3 model, rather than data curation and prompt hacking, contributes to our final results in semantic merge conflicts resolving, we conduct a user study to evaluate the difficulty of the resolution of semantic merge conflicts resolved by the GPT-3 model.
In detail, we provide the same input as we fed to GPT-3 to experienced developers and we ask them for the feasibility of the resolution.
A consensus conclusion has been made that if the resolution of semantic merge conflicts contains such a token that is not contained in the prompt, it is infeasible even for the expert to get the answer.

It is worth noticing that different than other text completion experiments that GPT-3 outputs tokens that are not in the prompt, in this experiment we assume that the resolution, if can be automatically learned, should be in the prompt.
This is because our prompt has conservatively collected all the changes that are related to the place that Clang complained at. 
It is also the situation that Edge developers face in everyday development.
Other sources of impreciseness could be introduced here, such as Clang pointed out the error to a wrong location, but this is rare.

We then automatically applied this as a filter to the model, and we found that in 286 “feasible” cases, GPT-3 gets the answer for 221 of them with the 77.3\% accuracy.
Surprisingly, in the “infeasible” category, among the rest of 93 examples, GPT-3 gets it in 14 times (15.1\%.) 
The details of our result is in Table~\ref{table:feasible}, which shows GPT-3 is able to generate complex fix.
\input{figs/feasibility}

Here is a challenging merge conflict example resolved by \app.
This shows \app is able to generate complex resolution that the previous AST-based method~\cite{SungLKCW20} was unable to handle.

{
\begin{figure}[!h]
    
\begin{lstlisting}[]
Question:
--web_app_info->app_url = url;
++web_app_info->start_url = url;

-web_app_info->app_url = url;

Answer:
+web_app_info->start_url = url;

Question:
...

--"request", permissions::PermissionRequestType::PERMISSION_NOTIFICATIONS,
++"request", permissions::RequestType::kNotifications, requesting_origin);

--permissions::PermissionRequestType request_type,
++permissions::RequestType request_type,

--permissions::PermissionRequestType::PERMISSION_NOTIFICATIONS) {
++if (request_type == permissions::RequestType::kNotifications) {

- case permissions::PermissionRequestType::PERMISSION_CAMERA_PAN_TILT_ZOOM:

Answer:
+ case permissions::RequestType::kCameraPanTiltZoom:
\end{lstlisting}
    \caption{A challenging merge conflict example resolved by \app.}
    \label{fig:challengingexample}
\end{figure}
}

\subsection{Evaluate \app on textual merge conflicts for a divergent fork}

In addition to solve non-textual merge conflicts, we applied \app on two challenging textual merge conflict problems to recognize the generality of our tool on resolving merge conflicts.

\para{Evaluate \app on the Edge Textual Merge Conflict Dataset} Problem of textual merge conflict resolution for header files and Macro in large projects has been studied in this paper~\cite{PanLNGLK21}. 

\if
Driven by the finding that many merge conflict solutions shared many repetitive patterns, the authors designed a new domain-specific language which captures the patterns from historical data as resolution strategies.
Applying the learned strategies to the new unseen merge conflict will automatically generate a resolution.
\fi

\para{Dataset Setup} To check whether \app could resolve header files and Macro related textual merge conflicts, we run \app on a Edge dataset publicly available at~\cite{PanLNGLK21}.

\input{figs/prose}

% Intro to what is the problem? why it is a challenging problem?

The dataset contains 162 Edge merge conflict examples. 
Each example has one to two lines of changes, and it is collected in an eight-week period (March 30 2020 to April 24, 2020). 
One such header file related merge conflict example is the following:
{
\begin{figure}[!h]
    
\begin{lstlisting}[escapechar=!]
Main branch(Chromium):
!\colorbox{pink!50}{- \#include ``ui/base/cursor/mojom/cursor\_type.mojom-shared.h'' }!
Forked Branch (Edge):
!\colorbox{green!10}{+ \#include ``ui/base/anonymous\_ui\_base\_features.h'' }!
!\colorbox{green!10}{+ \#include ``ui/base/mojom/cursor\_type.mojom-shared.h'' }!
\end{lstlisting}
    \caption{An Example of Merge Conflict Resolution by Removing a Duplicated Header. Line starting with a ``+'' means this line is kept in the final merged code. Lint starting with a ``-'' means this line is removed from the final merged code}
    \label{fig:edgeupstream}
\end{figure}
}
Since the file \lstinline{mojom-shared.h} is already defined in the downstream Edge repository, the developers deleted the \lstinline{mojom-shared.h} location from the main branch.



{
\begin{figure}[!h]
    
\begin{lstlisting}[escapechar=!]
Question:
<<<<<<< HEAD
#include "chrome/browser/ui/views/accessibility/caption_bubble_controller_views.h"'
=======
#include "chrome/browser/ui/views/accessibility/hc_with_theme_bubble_view.h"'
>>>>>>>

Answer:
#include "chrome/browser/ui/views/accessibility/caption_bubble_controller_views.h"
#include "chrome/browser/ui/views/accessibility/hc_with_theme_bubble_view.h"

Question:
<<<<<<< HEAD
#include "build/build_config.h"
=======
#include "media/media_buildflags.h"
>>>>>>>

Answer:
\end{lstlisting}
    \caption{An Example of Prompt in Textual Merge Conflict Resolution by \app}
    \label{fig:prose_gpt_example}
\end{figure}
}

Fig.~\ref{fig:prose_gpt_example} shows an example of our prompt to the GPT-3 model. We randomly selected the first five examples in the Header File datasets and two examples in the Macro datasets as the shots. For example, in Fig.~\ref{fig:prose_gpt_example}, line 1 to line 10 is our shot, which showed how a merge conflict is resolved by concatenating from two inputs. By feeding the shot to the GPT-3 model, it outputs:
\begin{lstlisting}
#include "build/build_config.h"
#include "media/media_buildflags.h"
\end{lstlisting}
and this is the exact resolution provided by the Edge developers.





%How does the shot look like? How do we design the shot?

%What is the result?



%may need to introduce what is the merge size
% what kind of problem this tool tried to solve

% Briefly introduce two datasets
% describe what is in the dataset? Why this dataset is a challenging benchmark? previous work cannot be applied on this work since this is not C++, so the AST-based method is no longer applicable.
% Table two 
% Accuracy for \app on the Deepmerge Dataset

\subsection{Evaluate \app on textual merge conflicts for a large number of JavaScript projects in GitHub.}
% Table three 

We also ran \app on the textual merge conflicts for a large number of JavaScript projects in GitHub.
We adopted the same datasets used by the previous work~\cite{dinella2021deepmerge}
% Accuracy for \app on the Prose Dataset

% mention the reason we do not have the best result in include dataset because it needs domain specific knowledge for the repository and this information is not contained and further inferred by just considering the dataset. ( Edge expert would know it. like logging.h
\input{figs/deepmerge}
This dataset contains thousands of merge conflict examples collected from Github.
Here is an example of real world example.
% waiting for the dataset

%Here is the prompt 


==> secs/motiv.tex <==
\section{Motivating Example}
\label{sec:motiv}
%We give here one more example to illustrate real merge conflict issues that downstream developers face in the daily development.
%In the example, \app automatically generates the resolution for developers to fix the merge conflict.

In this section we illustrate a complexity of real-world merge conflicts
that downstream developers face in the daily development. We closely 
inspect the example of a
broken build taken from the Edge repository. The compiler error message
only indicated that it could not find a definition for 
\lstinline{PermissionRequestType}. 

The correct resolution to this particular problem is
given in Fig.~\ref{fig:motiv_edgedownstream}. This was a repair that the 
developer has committed. However, this was also the solution that
\app instantly derives in a fully automated way: it states that the line 
annotated with - should 
be replaced with the line annotated with +.
{
\begin{figure}[!h]
    
\begin{lstlisting}[escapechar=!]
!\colorbox{pink!50}{- PermissionRequestType::PERMISSION\_CAMERA\_PAN\_TILT\_ZOOM:}!
!\colorbox{green!10}{+ RequestType::kCameraPanTiltZoom:}!
    
\end{lstlisting}
    \caption{A solution for the challenging semantic merge conflict resolution in Edge downstream.}
    \label{fig:motiv_edgedownstream}
\end{figure}
}

To correctly resolve a merge conflict, developers needs to learn how the upstream 
context changed and then apply the similar changes to the downstream context. 
To derive this particular resolution, it was not enough to find 
the relevant file in the commit history and then propagate the changes:
the developer needed to find three different files and manually combine 
the changes described in those files to derive 
the required resolution. We list the most
relevant changes in Fig.~\ref{fig:motiv_edgeupstream}.

{
\begin{figure}[!h]
    
\begin{lstlisting}[escapechar=!]
!\colorbox{pink!50}{- permissions::PermissionRequestType:: PERMISSION\_NOTIFICATIONS}!
!\colorbox{green!10}{+ permissions::RequestType::kNotifications}!

!\colorbox{pink!50}{- permissions::PermissionRequestType request\_type}!
!\colorbox{green!10}{+ permissions::RequestType request\_type}!

!\colorbox{pink!50}{- permissions::PermissionRequestType::PERMISSION\_NOTIFICATIONS)}!
!\colorbox{green!10}{+ if (request\_type == permissions::RequestType::kNotifications)}!



\end{lstlisting}
    \caption{Root cause of a challenging semantic merge conflict in Chromium upstream.}
    \label{fig:motiv_edgeupstream}
\end{figure}
}

The developers first detected that the root cause of this compiler error 
was due to fact that  \lstinline{PermissionRequestType} has been renamed 
to \lstinline{RequestType} in upstream.
However, applying these changes to the \lstinline{PermissionRequestType} 
downstream still did not resolve this merge conflict.
This was due to the fact that  
\lstinline{PERMISSION_NOTIFICATIONS} 
in upstream was changed to \lstinline{kNotifications}.
After the developer learned how the upstream context changed and applied 
the similar changes to the downstream context, the semantic merge conflict is resolved by changing
\lstinline{PERMISSION_CAMERA_PAN_TILT_ZOOM} to \lstinline{kCameraPanTiltZoom}.


The existing merge conflict resolution approaches~\cite{SungLKCW20,verbruggen2021semantic,PanLNGLK21} are not helpful in such cases, because their learning algorithms are limited 
when it comes to learning and combining complex string transformation.
Indeed, in our empirical evaluation, given in Sec.~\ref{subsec:semanticeval}, 
we show that none of our baseline methods could resolve this merge conflict. 
 

